Chain of Evidences and Evidence to Generate: Prompting for Context Grounded and Retrieval Augmented Reasoning

While chain-of-thoughts (CoT) prompting has revolutionized how LLMs perform reasoning tasks, its current methods and variations (e.g, Self-consistency, ReACT, Reflexion, Tree-of-Thoughts (ToT), Cumulative Reasoning (CR) etc.,) suffer from limitations like limited context grounding, hallucination/inconsistent output generation, and iterative sluggishness. To overcome these challenges, we introduce a novel mono/dual-step zero-shot prompting framework built upon two unique strategies Chain of Evidences (CoE)} and Evidence to Generate (E2G). Instead of unverified reasoning claims, our innovative approaches leverage the power of "evidence for decision making" by first focusing exclusively on the thought sequences explicitly mentioned in the context which then serve as extracted evidence, guiding the LLM's output generation process with greater precision and efficiency. This simple yet potent approach unlocks the full potential of chain-of-thoughts prompting, facilitating faster, more reliable, and contextually aware reasoning in LLMs. Our framework consistently achieves remarkable results across various knowledge-intensive reasoning and generation tasks, surpassing baseline approaches with state-of-the-art LLMs. For instance, (i) on the LogiQA benchmark using GPT-4, CoE achieves a new state-of-the-art accuracy of 53.8%, surpassing CoT by 18%, ToT by 11%, and CR by 9%; (ii) CoE with PaLM-2 outperforms the variable-shot performance of Gemini Ultra by 0.9 F1 points, achieving an F1 score of 83.3 on DROP. We release our prompts and outputs on these benchmarks as a new instruction tuning dataset for future research at https://huggingface.co/datasets/kagnlp/Chain-of-Evidences/.

==> sections/6_filter-granularity.tex <==

% \section{Ablations, Robustness \&  Limitations}
\label{sec:ablation}
% Our comprehensive studies w/ ablation experiments discussed above demonstrate both pros and cons of our framework.

 % While \tool robustly enhances CoT-like prompting and features a stronger context-aware and retrieval augmented reasoning regardless of tasks, benchmarks, LLMs, and settings as shown in Section \ref{sec:logiQA}-\ref{sec:exp:rag}, our experiments and ablations also reveal possible negativity for context-free reasoning and very long form generations as indicated in Section \ref{sec:e-step}, \ref{sec:best-parctice}, \ref{sec:exp:rag}. We conduct further ablations in following perspectives.
 
 While \tool effectively enhances CoT-like prompting, featuring a robustly improved context-aware and retrieval-augmented reasoning across various tasks, benchmarks, language models (LLMs), and settings, as demonstrated in Section \ref{sec:logiQA}-\ref{sec:exp:rag}, our comprehensive experiments and ablations also uncover potential shortcomings related to context-free reasoning and the generation of very long-form outputs, as highlighted in Section \ref{sec:e-step}, \ref{sec:best-parctice}, \ref{sec:exp:rag}. Further insights are gained through additional ablations from various perspectives.
 % \textbf{Cost:} While, a single step  \toolnospace-pro typically is more expressive, generic, and convenient, the 2-stepped \toolnospace-base can still be utilized as more cost-effectiveness as a whole as (i) prompts that dictates for step-by-step showcasing are usually more detailed, (ii) the output token costs are often higher than input tokens (iii) the G-step input context is the very short \emph{Evidence}.  \textbf{Failures: }
 % From ablations,  our known limitations include: (i) it still hallucinates (ii) overemphasising on grounding causes model failed to infer common sense, leveraging generic world knowledge, logic and principles (iii) another drawback that comes from  overemphasising on grounding is that model can generate "unknown", "can not be determined", "not mentioned in the context" type of answers more frequently than baseline CoT.  (examples on more categorical mistakes are in Appendix) \textbf{Drawbacks w.r.t CoT variants:}  In compare to iterative CoT variants (e.g., Reflexion), it may not enhance more even w/ more turns, it does not explore numerous paths like ToT and CR, and hence may significantly falls behind them where context-grounding is not required.
 % (v) on a small scale evaluation set, \tool significantly outperforms 2 rounds of CoT (EM>=2) which mainly analogous to the post-processing of G-step.
 \textbf{Cost:} While \toolnospace-pro demonstrates greater expressiveness and generality, when two-stepped prompting is applied (e.g., for long context), \toolnospace-base can still be more cost-effectiveness. This is evident due to the fact that (i) prompts requiring step-by-step demonstrations are often more detailed and output token costs typically exceed input token costs. (ii) the G-step input context is a concise \emph{Evidence}.
% \textbf{Failures:} Ablations reveal certain limitations of \tool, including (i) occasional hallucinations, (ii) an overemphasis on grounding leading to the model's failure to infer common sense, leverage generic world knowledge, logic, and principles, and (iii) a drawback associated with overemphasizing grounding, causing the model to generate responses such as "unknown," "cannot be determined," or "not mentioned in the context" more frequently than the baseline CoT. Specific examples of categorical mistakes are provided in the Appendix.
% \textbf{Drawbacks w.r.t CoT variants:} In comparison to iterative CoT variants (e.g., Reflexion), \tool may not exhibit significant improvement even with additional turns. It does not explore diverse paths like ToT and CR, and consequently, it may lag behind in scenarios where context-grounding is not a crucial requirement.

% \label{sec:neg:result-wow-eli5}

% \section{}

% We first introduce the experimental setup (\S\ref{sub:impl-detail}) and baseline approaches for comparison (\S\ref{sub:baseline}). Then, we evaluate model performance on both end generation (\S\ref{sub:gen-perf}) and context filtering (\S\ref{sub:filter-perf}). 



% cot or 2cot may work, mainly post-processing type of problem. 
% 2. qualitative example : general al thask
% 5. compare w/ cr?
% 6. retrieval er jonno kharap long form
% HotpotQa LLM even force to override given contetual info. 


% Negative: arithmatic (short cut khuje compuatation bipass kore)

% commonsense/general knowlfe ManU

% 1. Hotpotqa improve
% 2. Multi-agent (numerous coref)
% 2. Ablation: short precious evidence vs breadth space
% 3. Generic rterieval quality vs gain over CoT

% Idx 8783, 
% Qustion:  Brian De Palma is a writer.
% True ans:  ['SUPPORTS']
% e2g answer:  REFUTES
% e2g evidence:  The context does not mention that Brian De Palma is a writer.
%  cot answer:  SUPPORTS
%  evidence:  'The context states that Brian De Palma is a director.', 'The context also states that Brian De Palma is a graduate student in their theater department.', 'The co
% ntext also states that Brian De Palma is a composer.', 'Therefore, the claim that Brian De Palma is a writer is supported by the context.'
% limitations\href{}{
% Still hallucinate: Melbourne
% Joint Q, Long Q (no reason)
% unknown }

% Question:  Do The Importance of Being Icelandic and The Five Obstructions belong to different film genres ?
% Gold answer:  no
% cot ans:  {
%     "answer": "no",
%     "step_by_step_reasoning": "The Importance of Being Icelandic and The Five Obstructions are both documentary films, so they belong to the same film genre. Therefore, the $
% nswer is no."
% }
% Final reason:  {
%     "answer": "Cannot be determined",
%     "evidence_and_explanation": "The context does not provide any information about the genres of The Importance of Being Icelandic and The Five Obstructions. Therefore, it c
% annot be determined whether they belong to different film genres or not."
% }


% \subsection{Limitation}
% False/inaccurate reasonings:





==> sections/7_related-work.tex <==
\section{Related Work}
\label{sec:related-works}
% \paragraph{Augmented Generation}
% Providing additional contexts to generation has shown to be effective~\cite{lewis2020retrieval,guu2020realm,mialon2023augmented} across many knowledge-intensive tasks~\cite{petroni-etal-2021-kilt}. While the most common approach with a set of retrieved passages is to append them all to the input, some works explored the optimal granularity and strategy to do this.
% % optimal length
% \citet{wang-etal-2019-multi} identify 100 words to be the optimal size for candidate passages, which then became the \textit{de facto} length. Many works explored retrieval at varied granularity, including paragraph \citep{lee-etal-2019-latent,feldman-el-yaniv-2019-multi}, phrase \citep{lee-etal-2021-phrase}, and even token levels \citep{khandelwal2020generalization,alon2022neurosymbolic}, which all reveal a trade-off in difficulty between retrieval and generation: retrieving longer sequences is easier, but it is harder to generate correct output from them. 
% In fact, \citet{shi2023large} shows that model performance can dramatically decrease when irrelevant information is included in output-supporting documents. 
% Our method alleviates this in-passage distraction, by allowing arbitrary passage sizes at retrieval time, and providing precisely useful content for generation.

Various prompting paradigms have been studied in literature toward enhancing reasoning in LLMs. In Section \ref{sec:intro}, we provide
a (non-exhaustive) list of examples that employ the widely applied chain-of-thought techniques.  Among others,  search-based \citep{pryzant2023automatic, lu2021neurologic}, Program-aided LLM generation \citep{liu2023llm, gao2023pal, jung2022maieutic, zhu2022solving}, self generation of prompts \citep{he2023exploring, yasunaga2023large, sun2022recitation, kim2022self, li2022self}, self evaluation based approaches \citep{madaan2023self, xie2023decomposition, kim2023language, paul2023refiner} have been studied. 
Other works have also been extended w/ more complex multi-step reasoning procedure (e.g., using a different fine-tuned model \citep{zelikman2022star, nye2021show, lester-etal-2021-power}) or for domain specific applications \citep{parvez-etal-2023-retrieval, parvez-etal-2021-retrieval-augmented, ouyang2022training, sanh2021multitask, wei2021finetuned}. Closest to ours, \citet{creswell2022selection} adopts techniques that improves multi-stage reasoning where for each reasoning stage, it employs a two-agent (e.g., rationale selection and inference/premise derivation) method using k-shot annotated examples. Although this is beyond simple prompting, our approach constructively is a single-agent (same task/prompt) two-step 0-shot instruction guided prompting technique.  Nonetheless, while majority of existing works focus on context-free, arithmetic or commonsense reasoning, \tool uniquely tackles the context-aware reasoning reason more accurately and can be robustly applicable to tasks beyond reasoning (e.g. dialogue generation).


% A language model estimates probabilities over text. Recent research has scaled up these models from
% millions (Devlin et al., 2019) to billions of parameters (Brown et al., 2020) and expanded training data
% to include web texts and instruction data (Gao et al., 2020; Ouyang et al., 2022; Chung et al., 2022). These
% advances have made large language models proficient in various NLP tasks.
% LLMs with billions of parameters demonstrate in-context learning and few-shot learning abilities (Brown
% et al., 2020; Liu et al., 2022; Su et al., 2022; Mishra et al., 2022; Wei et al., 2022a; Yasunaga et al., 2023).
% They use input prompts (instructions or a few exemplars) to guide LLMs to generate desired responses
% for tasks, marking the advent of the prompting era. Our approach harnesses the in-context learning abilities
% of LLMs to guide their reasoning process using self-generated exemplars.
% Closely related to ours are works that perform self-generation in LLM prompting (Sun et al., 2022; He et al.,
% 2023; Kim et al., 2022; Li et al., 2022a). For instance, Sun et al. (2022) prompts LLMs to recite relevant
% facts in context for open-domain question answering. Our idea of self-generating exemplars is related to
% recitation, but focuses on recalling problem-solving and reasoning processes rather than factual knowledge.


% \paragraph{Optimizing Retrieval for Augmentation}
% Many works focus on post-process retrieved content to augment the generation.
% % passage reranking
% A common approach is to rerank retrieved passages and provide only the top few under limited input capacity, based on the similarity between query and passages \citep{nogueira2020passage}, the majority of reader predictions \citep{mao-etal-2021-reader}, and utility for generation \citep{wang2018r}.
% % \jun{There is a research topic called Answer Sentence Selection (AS2) in the context of question answering. I wonder if we can add one sentence to clarify how our work differs from prior work on the topic.}
% % optimal granularity
% \citet{asai-etal-2022-evidentiality} measures the evidentiality of retrieved passages to improve context quality, by removing irrelevant passages and skipping the retrieval step \citep{mallen2023trust}. Nonetheless, these methods operate on the coarse passage level, thus still suffering from in-passage distractions. 
% Our method has similarities to answer sentence selection \citep{yu2014deep}, which can operate at a more fine-grained sentence level. 
% Yet further, our filtering can apply to text split in arbitrary granularity that optimizes the task of interest, and capture more subtle variances in context.


==> sections/acknowledge.tex <==
\section*{Acknowledgements}

This work was supported in part by a grant from Bosch.
We thank the members of CMU LTI for their helpful discussion and feedback on this work.
